Implementing a unified solver for nonlinearly constrained optimization

SQP and interior-point methods (also referred to as Lagrange-Newton methods) typically share key algorithmic components, such as strategies for computing descent directions and mechanisms that promote global convergence. Building on this insight, we introduce a unifying framework with eight building blocks that abstracts the workflows of Lagrange-Newton methods. We then present Uno, a modular C++ solver that implements our unifying framework and allows the automatic combination of a wide range of strategies with no programming effort from the user. Uno is meant to (1) organize mathematical optimization strategies into a coherent hierarchy; (2) offer a wide range of efficient and robust methods that can be compared for a given instance; (3) enable researchers to experiment with novel optimization strategies; and (4) reduce the cost of development and maintenance of multiple optimization solvers. Uno's software design allows user to compose new customized solvers for emerging optimization areas such as robust optimization or optimization problems with complementarity constraints, while building on reliable nonlinear optimization techniques. We demonstrate that Uno is highly competitive against state-of-the-art solvers filterSQP, IPOPT, SNOPT, MINOS, LANCELOT, LOQO, and CONOPT on a subset of 429 small problems from the CUTE collection. Uno is available as open-source software under the MIT license at https://github.com/cvanaret/Uno and via its C, Julia, Python, Fortran, and AMPL interfaces.

==> sections/code_snippets.tex <==
\section{Code snippets}

\begin{landscape}
\inputminted[fontsize=\footnotesize]{cpp}{code/Uno.cpp}
\clearpage
\inputminted[fontsize=\footnotesize]{cpp}{code/TrustRegion.cpp}
\clearpage
\inputminted[fontsize=\footnotesize]{cpp}{code/LineSearch.cpp}
\end{landscape}


==> sections/combining_byrd.tex <==
\begin{algorithm}[htbp!]
\caption{Uno: line-search $\ell_1$-merit S$\ell_1$QP.}
\label{alg:uno-ls-merit-sl1qp}
\scriptsize
\SetAlgoVlined
\KwIn{initial primal-dual iterate $(x^{(0)}, \constraintmultipliers^{(0)}, \boundmultipliers^{(0)})$, initial penalty parameter $\rho$}
$k \gets 0$ \;
\begin{constraint_relaxation}
% progress measures/models
$(\infeasibilitymeasure(x), \objectivemeasure{\rho}(x), \highlight[subproblem_color]{\auxiliarymeasure(x)}) \equaldef (\| c(x) \|_1, \rho f(x), \highlight[subproblem_color]{0})$ \;
$(\Delta \infeasibilitymodel^{(k)}(\direction{x}), \Delta \objectivemodel{\rho}^{(k)}(\direction{x}), \highlight[subproblem_color]{\Delta \auxiliarymodel^{(k)}(\direction{x})}) \equaldef \Big( \| c^{(k)} \|_1 - \| c^{(k)} + (\nabla c^{(k)})^T \direction{x} \|_1, -\rho (\nabla f^{(k)})^T \direction{x}, \allowbreak \highlight[subproblem_color]{0} \Big)$ \;
\end{constraint_relaxation}
\begin{globalization_strategy}
% merit function and its local model
$\meritfunction{\rho} \equaldef \highlight[constraint_relaxation_color]{\objectivemeasure{\rho}} + \highlight[constraint_relaxation_color]{\infeasibilitymeasure} + \highlight[subproblem_color]{\auxiliarymeasure}$ \;
$\Delta \meritfunctionmodel{\rho}^{(k)} \equaldef \highlight[constraint_relaxation_color]{\Delta \objectivemodel{\rho}^{(k)}} + \highlight[constraint_relaxation_color]{\Delta \infeasibilitymodel^{(k)}} + \highlight[subproblem_color]{\Delta \auxiliarymodel^{(k)}}$ \;
\end{globalization_strategy}
   
\Repeat{termination criteria are satisfied} {
	\begin{globalization_mechanism}
   \begin{constraint_relaxation}
	$(\direction{x}^{(k)}, \direction{\constraintmultipliers}^{(k)}, \direction{\boundmultipliers}^{(k)}) \gets$ solve $(\ell_1 \highlight[subproblem_color]{QP}_\rho^{(k)})$ \;
	\If{$l^{(k)}(\direction{x}^{(k)}) > 0$} {
		$(\bar{\direction{x}}^{(k)}, \bar{\direction{\constraintmultipliers}}^{(k)}, \bar{\direction{\boundmultipliers}}^{(k)}) \gets$ solve $(\ell_1 \highlight[subproblem_color]{QP}_\rho^{(k)})$ with $\rho = 0$
        \Comment*[r]{Eq.~\eqref{eq:l1QP}}
		Decrease $\rho$ until the solution $(\direction{x}^{(k)}, \direction{\constraintmultipliers}^{(k)}, \direction{\boundmultipliers}^{(k)})$ to $(\ell_1 \highlight[subproblem_color]{QP}_\rho^{(k)})$ satisfies \;
		\begin{equation*}
		\begin{cases}
		l^{(k)}(\direction{x}^{(k)}) = 0					& \text{if } l^{(k)}(\bar{\direction{x}}^{(k)}) = 0 \\
		l^{(k)}(0) - l^{(k)}(\direction{x}^{(k)}) \ge \varepsilon_1 \left( l^{(k)}(0) - l^{(k)}(\bar{\direction{x}}^{(k)}) \right)	& \text{otherwise}
		\end{cases}
		\end{equation*}
		
		Further decrease $\rho$ until the solution $(\direction{x}^{(k)}, \direction{\constraintmultipliers}^{(k)}, \direction{\boundmultipliers}^{(k)})$ to $(\ell_1 \highlight[subproblem_color]{QP}_\rho^{(k)})$ satisfies \;
		$\highlight[strategy_color]{\Delta \meritfunctionmodel{\rho}^{(k)}}(\direction{x}^{(k)}) \ge \varepsilon_2 \highlight[strategy_color]{\Delta \meritfunctionmodel{0}^{(k)}}(\bar{\direction{x}}^{(k)})$
		
		$\rho \gets \min \left(\rho, \displaystyle\left( \frac{E_0^{(k)}(x^{(k)}, \constraintmultipliers^{(k)} + \bar{\direction{\constraintmultipliers}}^{(k)})}{\max \left(1, \| c(x^{(k)} \|_1) \right)}\right)^2 \right)$ \;
		\If{$\rho$ has decreased} {
			$(\direction{x}^{(k)}, \direction{\constraintmultipliers}^{(k)}, \direction{\boundmultipliers}^{(k)}) \gets$ solve $(\ell_1 \highlight[subproblem_color]{QP}_\rho^{(k)})$ \;
		}
	}
	\end{constraint_relaxation}
   
   $\alpha^{(0)} \gets 1$ \;
	Set inner iteration counter $l \gets 0$ \;
	\Repeat{$(\trial{x}^{(k+1,l)}, \trial{\constraintmultipliers}^{(k+1,l)}, \trial{\boundmultipliers}^{(k+1,l)})$ is acceptable} {
      Assemble trial iterate $(\trial{x}^{(k+1,l)}, \trial{\constraintmultipliers}^{(k+1,l)}, \trial{\boundmultipliers}^{(k+1,l)}) \equaldef (x^{(k)}, \constraintmultipliers^{(k)}, \boundmultipliers^{(k)}) + (\alpha^{(l)} \direction{x}^{(k)}, \alpha^{(l)} \direction{\constraintmultipliers}^{(k)}, \direction{\boundmultipliers}^{(k)})$ \;
      $\mathit{acceptable} \gets \mathit{false}$ \;
      
		\begin{constraint_relaxation}
      \eIf{$\|\direction{x}^{(k,l)}\| = 0$} {
			$\mathit{acceptable} \gets \mathit{true}$ \;
		}{
         \begin{globalization_strategy}
         % Armijo condition
         \If{$\meritfunction{\rho}(x^{(k)}) - \meritfunction{\rho}(\trial{x}^{(k+1, l)}) \ge \sigma \Delta \meritfunctionmodel{\rho}^{(k)}(\highlight[mechanism_color]{\alpha^{(l)}} \direction{x}^{(k)})$} {
            $\mathit{acceptable} \gets \mathit{true}$ \;
         }
         \end{globalization_strategy}
      }
		\end{constraint_relaxation}
		\If{not $\mathit{acceptable}$} {
			Decrease step length $\alpha^{(l)}$ \;
		}
		$l \gets l+1$ \;
	}
	Update $(x^{(k+1)}, \constraintmultipliers^{(k+1)}, \boundmultipliers^{(k+1)}) \gets (\trial{x}^{(k+1,l)}, \trial{\constraintmultipliers}^{(k+1,l)}, \trial{\boundmultipliers}^{(k+1,l)})$ \;
	\end{globalization_mechanism}
	$k \gets k+1$ \;
}
\Return $(x^{(k)}, \constraintmultipliers^{(k)}, \boundmultipliers^{(k)})$
\end{algorithm}


==> sections/combining_pseudo_codes.tex <==
\section{Combining the ingredients: pseudo-codes}

%\input{sections/combining_byrd}
\input{sections/combining_filtersqp}
\input{sections/combining_ipopt}


==> sections/sequence_diagrams.tex <==
%\subsection{Sequence diagrams}
%\label{sec:sequence-diagrams}

%In Figure~\ref{fig:sequence-diagrams}, we consider sequence diagrams\todo{Add reference!}, an alternative method for visualizing the interactions between the four ingredients in \uno{} . The vertical bars represent the different ingredients, and arrows indicate ... \todo{finish this description.}
%The sequence diagrams show the calling sequences between \uno{} classes for a line-search method and a trust-region method, respectively.

%\todo{write the TR sequence diagram in the same style as the LS diagram}

%\begin{figure}[htbp!]
    %\centering
    %\begin{subfigure}[b]{\columnwidth}
    %\centering
    %\includegraphics[width=0.85\textwidth]{sequence_diagrams/trust_region}
    %\caption{Trust-region strategy}
    %\end{subfigure}
    %\par\bigskip
    %\begin{subfigure}[b]{\columnwidth}
    %\centering
    %\includegraphics[width=0.85\textwidth]{sequence_diagrams/line_search}
    %\caption{Backtracking line search}
    %\end{subfigure}
    %\caption{\uno{}: sequence diagrams for two globalization mechanisms.}
    %\label{fig:sequence-diagrams}
%\end{figure}


==> sections/smooth_reformulation.tex <==
\section{Smooth reformulation of non-smooth $\ell_1$ problems}
\label{sec:smooth-reformulation}

The non-smooth $\ell_1$ problem
\begin{equation}
\begin{array}{ll} \dps
\mini_x	& a(x) + \|b(x)\|_1
\end{array}
\end{equation}
can be reformulated into a smooth problem with nonnegative elastic variables $\positiveelastic, \negativeelastic$ that capture the positive and negative parts of $b(x)$, respectively:

\begin{equation}
\begin{array}{lll} \dps
\mini_{x,\positiveelastic,\negativeelastic} & a(x) + e^T \positiveelastic + e^T \negativeelastic \\
\st 	& b(x) - \positiveelastic + \negativeelastic = 0 \\
		& \positiveelastic \ge 0, ~ \negativeelastic \ge 0,
\end{array}
\end{equation}
where $e$ is a vector of ones of appropriate size.
We note that introducing elastic variables makes the constraint Jacobian full rank, which ensures constraint qualification.


==> sections/statistics_table_constraints.tex <==
\begin{scriptsize}
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4pt}
\begin{longtable}{|c|ccc|ccccccc|}
\caption{Number of objective evaluations on a subset of linear CUTEst problems.}
\label{tab:statistics_linear_problems} \\
\hline
 & \multicolumn{3}{c|}{Uno presets}           & \multicolumn{7}{c|}{State-of-the-art solvers} \\
Problem & \texttt{filtersqp} & \texttt{ipopt} & \texttt{byrd} & filterSQP & IPOPT & SNOPT & MINOS & LANCELOT & LOQO & CONOPT \\
\hline
\endfirsthead
\hline
 & \multicolumn{3}{c|}{Uno presets}           & \multicolumn{7}{c|}{State-of-the-art solvers} \\
Problem & \texttt{filtersqp} & \texttt{ipopt} & \texttt{byrd} & filterSQP & IPOPT & SNOPT & MINOS & LANCELOT & LOQO & CONOPT \\
\hline
\endhead
booth & \textbf{1} & 2 & 2 & 3 & 2 & 2 & \textbf{1} & 3 & 7 & \textbf{1} \\
degenlpa & 2 & 27 & 3 & 3 & 29 & 26 & 15 & 25 & 29 & \textbf{1} \\
degenlpb & 2 & 29 & 3 & 3 & 41 & 26 & 23 & 45 & 30 & \textbf{1} \\
extrasim & 2 & 6 & 2 & 3 & 6 & \textbf{1} & \textbf{1} & 3 & 11 & \textbf{1} \\
goffin & 3 & 10 & 3 & 4 & 7 & 25 & 25 & 10 & 13 & \textbf{1} \\
himmelba & \textbf{1} & 2 & 2 & 3 & 2 & 2 & \textbf{1} & 3 & 7 & \textbf{1} \\
linspanh & 2 & 19 & 4 & 3 & 20 & 5 & 14 & 13 & 12 & \textbf{1} \\
makela4 & 3 & 9 & 2 & 4 & 8 & \textbf{1} & \textbf{1} & 20 & 12 & \textbf{1} \\
model & 2 & 16 & 3 & 3 & 30 & 23 & 34 & 33 & 15 & \textbf{1} \\
res & 3 & 9 & 2 & 3 & 10 & \textbf{1} & 5 & \textbf{1} & 12 & \textbf{1} \\
simpllpa & 2 & 14 & 2 & 3 & 14 & 3 & 3 & 5 & 12 & \textbf{1} \\
simpllpb & 2 & 12 & 2 & 3 & 11 & \textbf{1} & \textbf{1} & 4 & 13 & \textbf{1} \\
supersim & \textbf{1} & 3 & 2 & 3 & 2 & \textbf{1} & \textbf{1} & 7 & 11 & \textbf{1} \\
zangwil3 & \textbf{1} & 2 & 2 & 3 & 2 & 3 & 2 & 3 & 8 & \textbf{1} \\
\hline
\end{longtable}
\end{scriptsize}

\begin{scriptsize}
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4pt}
\begin{longtable}{|c|ccc|ccccccc|}
\caption{Number of objective evaluations on a subset of quadratic CUTEst problems.}
\label{tab:statistics_quadratic_problems} \\
\hline
 & \multicolumn{3}{c|}{Uno presets}           & \multicolumn{7}{c|}{State-of-the-art solvers} \\
Problem & \texttt{filtersqp} & \texttt{ipopt} & \texttt{byrd} & filterSQP & IPOPT & SNOPT & MINOS & LANCELOT & LOQO & CONOPT \\
\hline
\endfirsthead
\hline
 & \multicolumn{3}{c|}{Uno presets}           & \multicolumn{7}{c|}{State-of-the-art solvers} \\
Problem & \texttt{filtersqp} & \texttt{ipopt} & \texttt{byrd} & filterSQP & IPOPT & SNOPT & MINOS & LANCELOT & LOQO & CONOPT \\
\hline
\endhead
3pk & \textbf{1} & \textbf{1} & \textbf{1} & 7 & \textbf{1} & 41 & 95 & 47 & 20 & \textbf{1} \\
arglinb & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & \textbf{1} & 2 & 2 & 3 & \textbf{1} \\
arglinc & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & \textbf{1} & 2 & 2 & 3 & \textbf{1} \\
avgasa & \textbf{2} & 11 & 3 & 3 & 10 & 9 & 14 & 12 & 11 & 18 \\
avgasb & \textbf{2} & 14 & 3 & 3 & 13 & 9 & 11 & 11 & 16 & 21 \\
biggsc4 & \textbf{2} & 27 & 4 & 3 & 36 & 13 & 10 & 15 & 21 & 5 \\
bqp1var & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & \textbf{1} & \textbf{1} & 3 & 10 & \textbf{1} \\
bqpgabim & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & 36 & 54 & 6 & 14 & \textbf{1} \\
bqpgasim & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & 40 & 61 & 6 & 14 & \textbf{1} \\
bt3 & \textbf{2} & \textbf{2} & 3 & 3 & \textbf{2} & 5 & 4 & 6 & 3 & 8 \\
deconvb & \textbf{1} & -- & \textbf{1} & 30 & -- & 302 & 13 & 31 & 45 & \textbf{1} \\
dixon3dq & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & 10 & 19 & 4 & 3 & \textbf{1} \\
dual1 & \textbf{2} & 17 & 3 & 3 & 17 & 475 & -- & 9 & 22 & 29 \\
dual2 & \textbf{2} & 15 & 3 & 3 & 14 & 269 & -- & 9 & 19 & 27 \\
dual4 & \textbf{2} & 14 & 3 & 3 & 14 & 145 & -- & 8 & 21 & 23 \\
dualc1 & \textbf{2} & 29 & 3 & 3 & 58 & 7 & 11 & 17 & 26 & 14 \\
dualc2 & \textbf{2} & 27 & 3 & 3 & 54 & 5 & 6 & 19 & 21 & 17 \\
dualc5 & \textbf{2} & 11 & 3 & 3 & 11 & 7 & 11 & 8 & 16 & 15 \\
dualc8 & \textbf{2} & 14 & 3 & 3 & 26 & 9 & 13 & 24 & 19 & 25 \\
fccu & 4 & \textbf{2} & 4 & 5 & \textbf{2} & 19 & 23 & 13 & 3 & 10 \\
genhs28 & \textbf{2} & \textbf{2} & 3 & 3 & \textbf{2} & 11 & 4 & 5 & 3 & 8 \\
hatfldc & \textbf{1} & \textbf{1} & \textbf{1} & 5 & \textbf{1} & 16 & 9 & 9 & 9 & \textbf{1} \\
hatfldh & \textbf{2} & 15 & \textbf{2} & 3 & 19 & 3 & 3 & 13 & 16 & 5 \\
hilberta & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & 2 & 4 & 60 & 3 & \textbf{1} \\
hilbertb & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & 50 & -- & 5 & 3 & \textbf{1} \\
hs003 & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & 2 & 2 & 16 & 11 & \textbf{1} \\
hs021 & 2 & 8 & 3 & 2 & 9 & \textbf{1} & 2 & 3 & 12 & 12 \\
hs028 & \textbf{2} & \textbf{2} & 3 & \textbf{2} & \textbf{2} & 4 & 4 & 4 & 3 & 8 \\
hs035 & \textbf{2} & 9 & 3 & \textbf{2} & 8 & 5 & 5 & 8 & 10 & 12 \\
hs044 & \textbf{2} & 21 & 9 & \textbf{2} & 20 & \textbf{2} & \textbf{2} & 11 & 16 & 5 \\
hs048 & \textbf{2} & \textbf{2} & 3 & \textbf{2} & \textbf{2} & 6 & 7 & 3 & 3 & 9 \\
hs051 & \textbf{2} & \textbf{2} & 3 & \textbf{2} & \textbf{2} & 6 & 4 & 10 & 3 & 7 \\
hs052 & \textbf{2} & \textbf{2} & 3 & 3 & \textbf{2} & 5 & 4 & 6 & 3 & 8 \\
hs053 & \textbf{2} & 7 & 3 & 3 & 7 & \textbf{2} & 4 & 6 & 12 & 15 \\
hs054 & \textbf{2} & 8 & 3 & 3 & 8 & 5 & 6 & 9 & 12 & 11 \\
hs076 & \textbf{2} & 9 & 3 & \textbf{2} & 8 & 4 & 6 & 9 & 11 & 16 \\
hs118 & \textbf{3} & 13 & \textbf{3} & \textbf{3} & 12 & 21 & 21 & 19 & 17 & 4 \\
hs21mod & 2 & 17 & 3 & 2 & 17 & \textbf{1} & 2 & 3 & 20 & 12 \\
hs268 & \textbf{2} & 20 & 4 & \textbf{2} & 17 & 6 & 15 & 27 & 27 & 19 \\
hs35mod & 2 & 17 & 3 & 2 & 16 & \textbf{1} & \textbf{1} & 3 & 16 & 6 \\
hs3mod & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & 5 & 5 & 4 & 12 & \textbf{1} \\
hs44new & \textbf{2} & 15 & 5 & \textbf{2} & 14 & 4 & 4 & 10 & 21 & 4 \\
lotschd & \textbf{3} & 15 & 4 & 4 & 15 & 8 & 4 & 9 & 19 & 7 \\
lsqfit & \textbf{2} & 9 & 3 & \textbf{2} & 8 & 3 & 4 & 7 & 12 & 9 \\
maratosb & \textbf{1} & \textbf{1} & \textbf{1} & 13 & \textbf{1} & 4 & 2 & 8 & 21 & \textbf{1} \\
nasty & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & \textbf{1} & \textbf{1} & 5 & 3 & \textbf{1} \\
obstclal & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & 37 & 45 & 7 & 23 & \textbf{1} \\
obstclbl & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & 44 & 61 & 3 & 13 & \textbf{1} \\
obstclbu & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & 36 & 49 & 2 & 15 & \textbf{1} \\
oslbqp & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & 6 & 6 & 3 & 19 & \textbf{1} \\
palmer1c & \textbf{1} & \textbf{1} & \textbf{1} & 7 & \textbf{1} & 8 & 25 & 145 & -- & -- \\
palmer1d & \textbf{1} & \textbf{1} & \textbf{1} & 6 & \textbf{1} & 7 & 21 & 34 & -- & -- \\
palmer2c & \textbf{1} & \textbf{1} & \textbf{1} & 5 & \textbf{1} & 8 & 24 & 298 & -- & -- \\
palmer3c & \textbf{1} & \textbf{1} & \textbf{1} & 5 & \textbf{1} & 8 & 24 & 206 & -- & -- \\
palmer4c & \textbf{1} & \textbf{1} & \textbf{1} & 6 & \textbf{1} & 8 & 23 & 176 & -- & -- \\
palmer5c & \textbf{1} & \textbf{1} & \textbf{1} & 4 & \textbf{1} & 6 & 12 & 2 & -- & -- \\
palmer5d & \textbf{1} & \textbf{1} & \textbf{1} & 5 & \textbf{1} & 4 & 9 & 2 & -- & -- \\
palmer6c & \textbf{1} & \textbf{1} & \textbf{1} & 6 & \textbf{1} & 8 & 23 & 159 & -- & -- \\
palmer7c & \textbf{1} & \textbf{1} & \textbf{1} & 8 & \textbf{1} & 8 & 25 & 189 & -- & -- \\
palmer8c & \textbf{1} & \textbf{1} & \textbf{1} & 7 & \textbf{1} & 8 & 24 & 152 & -- & -- \\
portfl1 & \textbf{2} & 10 & 3 & \textbf{2} & 10 & 12 & 19 & 20 & 17 & 20 \\
portfl2 & \textbf{2} & 9 & 3 & \textbf{2} & 9 & 12 & 21 & 14 & 17 & 23 \\
portfl3 & \textbf{2} & 11 & 3 & \textbf{2} & 11 & 13 & 21 & 14 & 17 & 32 \\
portfl4 & \textbf{2} & 10 & 3 & \textbf{2} & 10 & 11 & 21 & 19 & 16 & 19 \\
portfl6 & \textbf{2} & 9 & 3 & \textbf{2} & 9 & 11 & 19 & 20 & 16 & 31 \\
qudlin & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & 11 & 11 & 2 & 20 & \textbf{1} \\
sim2bqp & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & 2 & 3 & 3 & 14 & \textbf{1} \\
simbqp & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & 2 & 4 & 2 & 13 & \textbf{1} \\
tame & \textbf{1} & 2 & 2 & 3 & 6 & \textbf{1} & 2 & 2 & 9 & 6 \\
tointqor & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & 50 & -- & 8 & 3 & \textbf{1} \\
zangwil2 & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & 2 & 4 & 4 & 3 & \textbf{1} \\
zecevic2 & \textbf{2} & 10 & 3 & \textbf{2} & 9 & \textbf{2} & 3 & 7 & 11 & 7 \\
\hline
\end{longtable}
\end{scriptsize}

\begin{scriptsize}
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4pt}
\begin{longtable}{|c|ccc|ccccccc|}
\caption{Number of objective evaluations on a subset of nonlinear CUTEst problems.}
\label{tab:statistics_nonlinear_problems} \\
\hline
 & \multicolumn{3}{c|}{Uno presets}           & \multicolumn{7}{c|}{State-of-the-art solvers} \\
Problem & \texttt{filtersqp} & \texttt{ipopt} & \texttt{byrd} & filterSQP & IPOPT & SNOPT & MINOS & LANCELOT & LOQO & CONOPT \\
\hline
\endfirsthead
\hline
 & \multicolumn{3}{c|}{Uno presets}           & \multicolumn{7}{c|}{State-of-the-art solvers} \\
Problem & \texttt{filtersqp} & \texttt{ipopt} & \texttt{byrd} & filterSQP & IPOPT & SNOPT & MINOS & LANCELOT & LOQO & CONOPT \\
\hline
\endhead
aircrfta & \textbf{4} & \textbf{4} & \textbf{4} & \textbf{4} & \textbf{4} & -- & 9 & 10 & 6 & 7 \\
aircrftb & \textbf{1} & \textbf{1} & \textbf{1} & 21 & \textbf{1} & 112 & 30 & 27 & 21 & \textbf{1} \\
airport & 13 & 17 & \textbf{10} & 13 & 16 & 58 & 526 & 69 & 19 & 919 \\
aljazzaf & 21 & -- & 40 & \textbf{19} & 82 & 145 & 63 & 24 & 79 & 656 \\
allinitc & 28 & 45 & \textbf{14} & 24 & 44 & 105 & 54 & 76 & -- & 27 \\
allinit & \textbf{1} & \textbf{1} & \textbf{1} & 11 & \textbf{1} & 15 & 11 & 13 & 18 & \textbf{1} \\
allinitu & \textbf{1} & \textbf{1} & \textbf{1} & 12 & \textbf{1} & 13 & 9 & 15 & 11 & \textbf{1} \\
alsotame & \textbf{5} & 9 & \textbf{5} & \textbf{5} & 9 & 6 & 10 & 11 & 11 & 13 \\
argauss & \textbf{3} & -- & \textbf{3} & 7 & -- & 10 & -- & -- & -- & 5 \\
avion2 & 23 & 78 & \textbf{3} & 20 & 162 & 44 & 9 & 787 & 65 & 25 \\
bard & \textbf{1} & \textbf{1} & \textbf{1} & 11 & \textbf{1} & 26 & 13 & 15 & 19 & \textbf{1} \\
batch & 9 & 32 & \textbf{8} & 10 & 68 & 33 & 378 & -- & 64 & 277 \\
beale & \textbf{1} & \textbf{1} & \textbf{1} & 10 & \textbf{1} & 15 & 9 & 21 & 10 & \textbf{1} \\
biggs3 & \textbf{1} & \textbf{1} & \textbf{1} & 11 & \textbf{1} & 24 & 13 & 40 & 12 & \textbf{1} \\
biggs5 & \textbf{1} & \textbf{1} & \textbf{1} & 50 & \textbf{1} & 139 & 16 & 64 & 32 & \textbf{1} \\
biggs6 & \textbf{1} & \textbf{1} & \textbf{1} & 83 & \textbf{1} & 163 & 48 & 103 & 59 & \textbf{1} \\
box2 & \textbf{1} & \textbf{1} & \textbf{1} & 9 & \textbf{1} & 6 & 3 & 20 & 10 & \textbf{1} \\
box3 & \textbf{1} & \textbf{1} & \textbf{1} & 8 & \textbf{1} & 23 & 6 & 31 & 11 & \textbf{1} \\
brkmcc & \textbf{1} & \textbf{1} & \textbf{1} & 4 & \textbf{1} & 7 & 5 & 7 & 8 & \textbf{1} \\
brownal & \textbf{1} & \textbf{1} & \textbf{1} & 8 & \textbf{1} & 24 & 36 & 24 & 10 & \textbf{1} \\
brownbs & \textbf{1} & \textbf{1} & \textbf{1} & 48 & \textbf{1} & 49 & 10 & 7 & 49 & \textbf{1} \\
brownden & \textbf{1} & \textbf{1} & \textbf{1} & 9 & \textbf{1} & 76 & 15 & 9 & 57 & \textbf{1} \\
bt10 & \textbf{7} & 8 & \textbf{7} & \textbf{7} & \textbf{7} & 24 & 12 & 20 & 11 & 23 \\
bt11 & \textbf{7} & 9 & 8 & 8 & 9 & 12 & 55 & 22 & 11 & 20 \\
bt12 & \textbf{5} & \textbf{5} & \textbf{5} & \textbf{5} & \textbf{5} & 10 & 58 & 11 & 11 & 50 \\
bt13 & \textbf{18} & 25 & 24 & 50 & 25 & 34 & 208 & -- & 21 & 4060 \\
bt1 & \textbf{1} & 15 & \textbf{1} & 2 & 16 & 12 & 15 & 19 & 24 & \textbf{1} \\
bt2 & \textbf{13} & \textbf{13} & \textbf{13} & \textbf{13} & \textbf{13} & 18 & 384 & 36 & 18 & 220 \\
bt4 & \textbf{8} & 11 & 14782 & 12 & 12 & 10 & 47 & 25 & 9 & 84 \\
bt5 & 9 & \textbf{8} & 27 & 10 & \textbf{8} & 11 & 171 & 20 & \textbf{8} & 113 \\
bt6 & \textbf{11} & \textbf{11} & 31 & 12 & 18 & 14 & 116 & 25 & 12 & 126 \\
bt7 & 21 & 26 & 62 & 19 & 30 & 36 & 84 & 49 & \textbf{18} & 184 \\
bt8 & \textbf{12} & 29 & 31 & \textbf{12} & 15 & 14 & 20 & 30 & -- & 41 \\
bt9 & 25 & \textbf{14} & 40 & 29 & \textbf{14} & 29 & 79 & 22 & \textbf{14} & 216 \\
byrdsphr & 23 & 28 & 56 & 13 & 29 & 201 & 98 & 43 & \textbf{11} & 254 \\
camel6 & \textbf{1} & \textbf{1} & \textbf{1} & 8 & \textbf{1} & 15 & 8 & 8 & 12 & \textbf{1} \\
cantilvr & 13 & 13 & 18 & 18 & \textbf{12} & 28 & 177 & 27 & 16 & 325 \\
catena & 12 & \textbf{7} & 16 & 13 & \textbf{7} & 146 & 419 & 56 & 26 & 500 \\
cb2 & \textbf{7} & 10 & \textbf{7} & \textbf{7} & 9 & 13 & 79 & 18 & 11 & 51 \\
cb3 & \textbf{7} & 11 & \textbf{7} & \textbf{7} & 10 & 17 & 73 & 18 & 11 & 34 \\
chaconn1 & \textbf{5} & 8 & \textbf{5} & \textbf{5} & 7 & 13 & 56 & 12 & 11 & 28 \\
chaconn2 & \textbf{5} & 8 & \textbf{5} & \textbf{5} & 7 & 8 & 56 & 11 & 11 & 7 \\
chebyqad & \textbf{1} & \textbf{1} & \textbf{1} & 50 & \textbf{1} & -- & -- & 62 & 12 & \textbf{1} \\
chnrosnb & \textbf{1} & \textbf{1} & \textbf{1} & 59 & \textbf{1} & 230 & -- & 68 & 58 & \textbf{1} \\
cliff & \textbf{1} & \textbf{1} & \textbf{1} & 28 & \textbf{1} & 27 & 9 & 28 & 32 & \textbf{1} \\
cluster & 10 & 10 & \textbf{9} & 10 & 10 & -- & 23 & 45 & 11 & 150 \\
concon & 15 & 10 & \textbf{6} & 8 & 10 & 9 & -- & 676 & -- & 444 \\
congigmz & 6 & 34 & 7 & \textbf{5} & 33 & 24 & 44 & 30 & 36 & 188 \\
coolhans & \textbf{3} & 10 & -- & 4 & 10 & -- & 8 & 281 & 25 & 38 \\
core1 & 238 & -- & -- & 14 & 172 & \textbf{13} & 152 & -- & 52 & 756 \\
coshfun & 86 & -- & -- & 303 & -- & 234 & 2509 & 154 & \textbf{24} & 957 \\
cresc4 & 69 & 190 & -- & \textbf{59} & 80 & 93 & 863 & -- & 111 & 384 \\
csfi1 & 15 & \textbf{13} & 88 & 18 & 24 & 49 & -- & 155 & 16 & 54 \\
csfi2 & 52 & 332 & -- & \textbf{11} & 172 & 85 & -- & 180 & 17 & 17 \\
cube & \textbf{1} & \textbf{1} & \textbf{1} & 41 & \textbf{1} & 46 & 23 & 52 & 41 & \textbf{1} \\
dallass & \textbf{18} & 23 & 77 & 57 & 29 & 138 & 69 & -- & -- & -- \\
deconvc & 24 & 73 & \textbf{12} & 58 & 99 & 81 & 86 & 43 & 31 & 116 \\
deconvu & \textbf{1} & \textbf{1} & \textbf{1} & 971 & \textbf{1} & 238 & 13 & 69 & 76 & \textbf{1} \\
demymalo & \textbf{8} & 13 & 16 & 9 & 12 & 19 & 96 & 28 & 15 & 108 \\
denschna & \textbf{1} & \textbf{1} & \textbf{1} & 7 & \textbf{1} & 11 & 8 & 13 & 9 & \textbf{1} \\
denschnb & \textbf{1} & \textbf{1} & \textbf{1} & 10 & \textbf{1} & 10 & 8 & 11 & 9 & \textbf{1} \\
denschnc & \textbf{1} & \textbf{1} & \textbf{1} & 11 & \textbf{1} & 21 & 13 & 13 & 14 & \textbf{1} \\
denschnd & \textbf{1} & \textbf{1} & \textbf{1} & 43 & \textbf{1} & 144 & 39 & 65 & 44 & \textbf{1} \\
denschne & \textbf{1} & \textbf{1} & \textbf{1} & 11 & \textbf{1} & 42 & 10 & 16 & 15 & \textbf{1} \\
denschnf & \textbf{1} & \textbf{1} & \textbf{1} & 7 & \textbf{1} & 11 & 8 & 8 & 11 & \textbf{1} \\
dipigri & \textbf{12} & 19 & 19 & 13 & 22 & 23 & 128 & 63 & \textbf{12} & 165 \\
disc2 & \textbf{17} & 49 & 253 & 183 & 96 & 523 & -- & -- & 28 & 1266 \\
discs & 7459 & -- & -- & \textbf{41} & 426 & -- & -- & 422 & 59 & 1696 \\
dixchlng & \textbf{10} & 11 & -- & 12 & 11 & 31 & -- & 44 & 26 & 294 \\
djtl & \textbf{1} & \textbf{1} & \textbf{1} & 29 & \textbf{1} & -- & -- & 100 & 132 & \textbf{1} \\
dnieper & \textbf{4} & 31 & 594 & \textbf{4} & 31 & 13 & 35 & 75 & 25 & 29 \\
eg1 & \textbf{1} & \textbf{1} & \textbf{1} & 8 & \textbf{1} & 9 & 5 & 9 & 10 & \textbf{1} \\
eigencco & 20 & \textbf{13} & 21 & 29 & 14 & 34 & 157 & 17 & 22 & 130 \\
eigmaxc & \textbf{6} & 9 & 10 & 7 & 7 & 12 & -- & 21 & 14 & 22 \\
eigminc & \textbf{6} & 12 & 12 & 8 & 8 & 11 & 121 & 11 & 13 & 23 \\
engval2 & \textbf{1} & \textbf{1} & \textbf{1} & 20 & \textbf{1} & 44 & 22 & 30 & 28 & \textbf{1} \\
errinros & \textbf{1} & \textbf{1} & \textbf{1} & 53 & \textbf{1} & 519 & -- & 76 & 60 & \textbf{1} \\
expfita & 13 & 35 & 19 & 13 & 31 & 43 & \textbf{10} & 54 & 23 & 14 \\
expfit & \textbf{1} & \textbf{1} & \textbf{1} & 13 & \textbf{1} & 12 & 9 & 11 & 13 & \textbf{1} \\
extrosnb & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} \\
fletcher & \textbf{1} & 27 & 12 & 3 & 56 & 2 & -- & 28 & 14 & 224 \\
genhumps & \textbf{1} & \textbf{1} & \textbf{1} & 188 & \textbf{1} & 60 & 57 & 134 & 146 & \textbf{1} \\
gigomez1 & \textbf{8} & 19 & 17 & 9 & 19 & 18 & 142 & 33 & 16 & 74 \\
gottfr & 31 & \textbf{8} & \textbf{8} & 13 & 9 & -- & 11 & 35 & 12 & 121 \\
gridnetg & \textbf{4} & 16 & 5 & 5 & 11 & 48 & 23 & 21 & 12 & 21 \\
gridneth & \textbf{5} & 9 & \textbf{5} & 6 & 7 & 115 & 55 & 20 & 12 & 12 \\
gridneti & \textbf{5} & 14 & \textbf{5} & 6 & 14 & 121 & 56 & 22 & 16 & 24 \\
growthls & \textbf{1} & \textbf{1} & -- & 106 & \textbf{1} & 289 & 100 & 178 & 122 & \textbf{1} \\
growth & \textbf{1} & \textbf{1} & -- & 106 & \textbf{1} & 295 & 98 & 178 & 143 & \textbf{1} \\
gulf & \textbf{1} & \textbf{1} & \textbf{1} & 26 & \textbf{1} & 124 & 277 & 63 & 26 & \textbf{1} \\
hadamals & \textbf{1} & \textbf{1} & \textbf{1} & 13 & \textbf{1} & 289 & 167 & 20 & 13 & \textbf{1} \\
haifas & 12 & 11 & 58 & 13 & \textbf{10} & 24 & 145 & 27 & 13 & 42 \\
hairy & \textbf{1} & \textbf{1} & \textbf{1} & 84 & \textbf{1} & 21 & 13 & 102 & 64 & \textbf{1} \\
haldmads & 18 & -- & 85 & 42 & 103 & \textbf{13} & 130 & 45 & 31 & 175 \\
hart6 & \textbf{1} & \textbf{1} & \textbf{1} & 11 & \textbf{1} & 22 & 14 & 9 & 23 & \textbf{1} \\
hatflda & \textbf{1} & \textbf{1} & \textbf{1} & 15 & \textbf{1} & 32 & 20 & 47 & 9 & \textbf{1} \\
hatfldb & \textbf{1} & \textbf{1} & \textbf{1} & 11 & \textbf{1} & 31 & 14 & 28 & 11 & \textbf{1} \\
hatfldd & \textbf{1} & \textbf{1} & \textbf{1} & 23 & \textbf{1} & 29 & 20 & 66 & 25 & \textbf{1} \\
hatflde & \textbf{1} & \textbf{1} & \textbf{1} & 26 & \textbf{1} & 34 & 22 & 57 & 29 & \textbf{1} \\
hatfldf & 23 & -- & 2682 & 15 & 1594 & -- & \textbf{13} & 113 & \textbf{13} & 275 \\
hatfldg & 18 & 20 & 70 & 25 & 22 & -- & \textbf{12} & 29 & 16 & 155 \\
heart6ls & \textbf{1} & \textbf{1} & \textbf{1} & -- & \textbf{1} & -- & -- & -- & -- & \textbf{1} \\
heart6 & 199 & 1516 & 2845 & 133 & \textbf{75} & -- & 130 & -- & 327 & 1205 \\
heart8ls & \textbf{1} & \textbf{1} & \textbf{1} & 217 & \textbf{1} & -- & 215 & 238 & 108 & \textbf{1} \\
heart8 & 146 & 37 & 117 & \textbf{28} & 44 & -- & -- & 359 & 39 & 911 \\
helix & \textbf{1} & \textbf{1} & \textbf{1} & 19 & \textbf{1} & 35 & 25 & 18 & 13 & \textbf{1} \\
himmelbb & \textbf{1} & \textbf{1} & \textbf{1} & 25 & \textbf{1} & 6 & 4 & 11 & 16 & \textbf{1} \\
himmelbc & \textbf{7} & 8 & \textbf{7} & 8 & 9 & -- & 10 & 11 & 8 & 56 \\
himmelbd & 10 & -- & 23 & \textbf{7} & 83 & 28 & -- & -- & -- & 107 \\
himmelbe & \textbf{2} & 3 & 4 & 3 & 3 & -- & 4 & 8 & 8 & \textbf{2} \\
himmelbf & \textbf{1} & \textbf{1} & \textbf{1} & 8 & \textbf{1} & 105 & 20 & 29 & 24 & \textbf{1} \\
himmelbg & \textbf{1} & \textbf{1} & \textbf{1} & 10 & \textbf{1} & 11 & 7 & 16 & 7 & \textbf{1} \\
himmelbh & \textbf{1} & \textbf{1} & \textbf{1} & 8 & \textbf{1} & 9 & 3 & 7 & 9 & \textbf{1} \\
himmelbk & \textbf{6} & 19 & 573 & 7 & 19 & 12 & 173 & 206 & 23 & 178 \\
himmelp1 & \textbf{1} & \textbf{1} & \textbf{1} & 9 & \textbf{1} & 15 & 5 & 29 & 11 & \textbf{1} \\
himmelp2 & \textbf{9} & 22 & 10 & \textbf{9} & 19 & 32 & 150 & 275 & 20 & 143 \\
himmelp3 & \textbf{4} & 10 & \textbf{4} & 5 & 13 & 8 & 118 & 870 & 17 & 22 \\
himmelp4 & \textbf{4} & 12 & 5 & 5 & 25 & 8 & 114 & 737 & 17 & 31 \\
himmelp5 & \textbf{11} & 27 & 15 & 12 & 158 & 44 & 74 & 273 & 90 & 113 \\
himmelp6 & \textbf{1} & 12 & \textbf{1} & 2 & 12 & 2 & 4 & 2 & 45 & \textbf{1} \\
hong & \textbf{4} & 13 & 7 & 6 & 13 & 7 & 6 & 6 & 20 & 5 \\
hs001 & \textbf{1} & \textbf{1} & \textbf{1} & 36 & \textbf{1} & 63 & 3 & 41 & 35 & \textbf{1} \\
hs002 & \textbf{1} & \textbf{1} & \textbf{1} & 9 & \textbf{1} & 16 & 4 & 7 & 21 & \textbf{1} \\
hs004 & \textbf{1} & \textbf{1} & \textbf{1} & 3 & \textbf{1} & 2 & 2 & 2 & 8 & \textbf{1} \\
hs005 & \textbf{1} & \textbf{1} & \textbf{1} & 11 & \textbf{1} & 8 & 6 & 9 & 10 & \textbf{1} \\
hs006 & \textbf{3} & 8 & 12 & \textbf{3} & 7 & 9 & 90 & 63 & 10 & 4 \\
hs007 & 12 & 51 & \textbf{11} & 13 & 58 & 30 & 64 & 26 & 12 & 128 \\
hs008 & \textbf{6} & \textbf{6} & \textbf{6} & \textbf{6} & \textbf{6} & -- & 9 & 13 & 8 & 23 \\
hs009 & 5 & 5 & 5 & 5 & 6 & 9 & \textbf{2} & 22 & 9 & 8 \\
hs010 & \textbf{10} & 14 & 26 & \textbf{10} & 13 & 32 & 60 & 18 & 15 & 166 \\
hs011 & \textbf{6} & 10 & \textbf{6} & \textbf{6} & 9 & 15 & 45 & 16 & 12 & 11 \\
hs012 & \textbf{8} & 10 & 9 & \textbf{8} & 9 & 11 & 157 & 26 & 11 & 43 \\
hs013 & 25 & 1084 & 22 & 34 & 78 & \textbf{17} & 52 & 60 & -- & 113 \\
hs014 & \textbf{6} & 9 & \textbf{6} & 7 & 16 & 10 & 8 & 13 & 11 & 26 \\
hs015 & 6 & 22 & 8 & 7 & 21 & 11 & 84 & 47 & 31 & \textbf{5} \\
hs016 & \textbf{5} & 11 & 6 & \textbf{5} & 23 & \textbf{5} & 8 & 19 & 18 & 14 \\
hs017 & \textbf{8} & 21 & 9 & \textbf{8} & 18 & 19 & 10 & 20 & 30 & 33 \\
hs018 & \textbf{7} & 15 & \textbf{7} & \textbf{7} & 27 & 32 & 92 & 117 & 15 & 202 \\
hs019 & 7 & 17 & \textbf{6} & 7 & 16 & 9 & 55 & 45 & 18 & 37 \\
hs020 & \textbf{5} & 9 & \textbf{5} & \textbf{5} & 7 & \textbf{5} & 7 & 23 & 24 & 9 \\
hs022 & \textbf{1} & 8 & 5 & 3 & 7 & 7 & 46 & 10 & 9 & 18 \\
hs023 & \textbf{7} & 12 & \textbf{7} & \textbf{7} & 12 & \textbf{7} & 52 & 51 & 18 & 41 \\
hs024 & 2 & 12 & 16 & 3 & 12 & 5 & \textbf{1} & 14 & 13 & 3 \\
hs025 & \textbf{1} & \textbf{1} & \textbf{1} & 27 & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & 20 & \textbf{1} \\
hs026 & 18 & 26 & 19 & 18 & 26 & 27 & 75 & 41 & \textbf{14} & 149 \\
hs027 & 25 & -- & 1050 & \textbf{8} & 156 & 21 & 135 & 31 & 16 & 42 \\
hs029 & \textbf{8} & 10 & 25 & \textbf{8} & 9 & 14 & 172 & 18 & 10 & 73 \\
hs030 & \textbf{2} & 25 & 3 & \textbf{2} & 26 & 5 & 28 & 8 & 9 & 85 \\
hs031 & \textbf{6} & 9 & \textbf{6} & \textbf{6} & 8 & 11 & 27 & 12 & 17 & 125 \\
hs032 & \textbf{2} & 17 & 3 & \textbf{2} & 40 & 5 & 13 & 7 & 24 & 8 \\
hs033 & \textbf{5} & 12 & 16 & \textbf{5} & 16 & 9 & 38 & 9 & 11 & 15 \\
hs034 & \textbf{8} & 11 & 14 & \textbf{8} & 10 & \textbf{8} & 34 & 21 & 15 & 101 \\
hs036 & \textbf{2} & 14 & 6 & 3 & 13 & 10 & 3 & 7 & 20 & 3 \\
hs037 & \textbf{6} & 14 & 81 & \textbf{6} & 13 & 11 & 8 & 13 & 11 & 15 \\
hs038 & \textbf{1} & \textbf{1} & \textbf{1} & 54 & \textbf{1} & 141 & 33 & 56 & 13 & \textbf{1} \\
hs039 & 25 & \textbf{14} & 40 & 29 & \textbf{14} & 29 & 79 & 22 & \textbf{14} & 216 \\
hs040 & 5 & \textbf{4} & 23 & 5 & \textbf{4} & 9 & 20 & 11 & 8 & 32 \\
hs041 & \textbf{1} & 9 & 44 & 3 & 12 & 9 & \textbf{1} & 7 & 16 & 14 \\
hs042 & \textbf{6} & 7 & \textbf{6} & \textbf{6} & 7 & 10 & 20 & 13 & 9 & 91 \\
hs043 & 9 & 11 & \textbf{8} & 11 & 10 & 11 & 101 & 25 & 12 & 183 \\
hs045 & \textbf{1} & \textbf{1} & \textbf{1} & 2 & \textbf{1} & \textbf{1} & \textbf{1} & \textbf{1} & 25 & \textbf{1} \\
hs046 & 19 & 20 & \textbf{18} & 19 & 20 & 32 & 120 & 28 & \textbf{18} & 115 \\
hs047 & 21 & 25 & \textbf{19} & 21 & 21 & 28 & 124 & 29 & 24 & 141 \\
hs049 & \textbf{17} & 20 & 19 & \textbf{17} & 20 & 38 & 25 & 38 & 21 & 21 \\
hs050 & \textbf{9} & 10 & 10 & \textbf{9} & 10 & 24 & 10 & 11 & 16 & 14 \\
hs055 & 2 & 8 & 2 & 3 & 4 & 3 & 2 & 7 & 11 & \textbf{1} \\
hs056 & 16 & 35 & 114 & 19 & 39 & 52 & 51 & \textbf{12} & \textbf{12} & 154 \\
hs057 & 5 & 25 & 26 & 5 & 28 & -- & 27 & \textbf{2} & 14 & 86 \\
hs059 & 12 & 183 & 14 & \textbf{11} & 72 & 22 & 126 & 340 & 27 & 178 \\
hs060 & \textbf{7} & 8 & \textbf{7} & \textbf{7} & 8 & 13 & 119 & 18 & 9 & 120 \\
hs061 & \textbf{2} & 30 & 6 & \textbf{2} & 10 & 39 & 69 & 19 & 10 & \textbf{2} \\
hs062 & 8 & 9 & \textbf{7} & 11 & 9 & 13 & \textbf{7} & 37 & 13 & 19 \\
hs063 & 10 & 8 & 22 & \textbf{3} & 8 & 18 & 118 & 21 & 8 & 80 \\
hs064 & 17 & 19 & 74 & \textbf{16} & 18 & 28 & 97 & 38 & 26 & 149 \\
hs065 & \textbf{5} & -- & \textbf{5} & \textbf{5} & 91 & 11 & 318 & 42 & 19 & 89 \\
hs066 & 9 & 8 & 9 & 14 & 8 & \textbf{7} & 22 & 11 & 15 & 65 \\
hs067 & 12 & 12 & \textbf{2} & 13 & 12 & 32 & 59 & 287 & 17 & 111 \\
hs070 & 40 & \textbf{13} & 25 & 42 & 36 & 34 & 65 & 39 & 23 & 31 \\
hs071 & \textbf{6} & 10 & 48 & \textbf{6} & 18 & 8 & 54 & 16 & 13 & 70 \\
hs072 & 18 & 18 & 211 & 22 & \textbf{17} & 36 & 154 & 65 & 28 & 131 \\
hs073 & 4 & 11 & \textbf{3} & 5 & 18 & 8 & 17 & 18 & 21 & 18 \\
hs074 & 26 & \textbf{11} & 29 & \textbf{11} & 20 & 15 & 26 & 13 & 16 & 58 \\
hs075 & 25 & 11 & 20 & \textbf{10} & 20 & 12 & 17 & 110 & 18 & 31 \\
hs077 & \textbf{11} & \textbf{11} & 12 & 14 & 13 & 16 & 122 & 27 & 12 & 94 \\
hs078 & \textbf{5} & \textbf{5} & 36 & \textbf{5} & \textbf{5} & 7 & 56 & 12 & 8 & 46 \\
hs079 & \textbf{5} & \textbf{5} & \textbf{5} & \textbf{5} & \textbf{5} & 12 & 53 & 14 & 7 & 129 \\
hs080 & 8 & \textbf{7} & 8 & 8 & \textbf{7} & 9 & 47 & 13 & 10 & 90 \\
hs081 & 29 & \textbf{8} & -- & 38 & \textbf{8} & 11 & 54 & 17 & 16 & 90 \\
hs083 & 5 & 18 & \textbf{4} & 5 & 15 & 8 & 10 & 16 & 14 & 27 \\
hs084 & 10 & 13 & -- & \textbf{6} & 12 & 58 & 44 & 47 & 44 & 11 \\
hs085 & 62 & -- & 74 & -- & 143 & -- & -- & -- & 63 & \textbf{27} \\
hs086 & 5 & 14 & \textbf{4} & 5 & 11 & 29 & 7 & 15 & 13 & 19 \\
hs087 & 10 & 18 & 33 & \textbf{9} & 18 & 12 & 52 & 32 & 25 & 52 \\
hs088 & 28 & 28 & 63 & 22 & \textbf{18} & 59 & 65 & 56 & 27 & 568 \\
hs089 & 31 & 29 & \textbf{22} & 31 & 38 & 85 & 196 & 61 & 30 & 1023 \\
hs090 & 61 & 23 & 14 & \textbf{3} & 28 & 55 & 91 & 58 & 29 & 695 \\
hs091 & 111 & 16 & 23 & 337 & \textbf{15} & 73 & 214 & 62 & 28 & 903 \\
hs092 & 89 & 23 & 26 & \textbf{3} & 25 & 56 & 109 & 58 & 22 & 1027 \\
hs093 & \textbf{2} & 12 & 1619 & 3 & 10 & 33 & -- & -- & 13 & 136 \\
hs095 & \textbf{2} & 17 & \textbf{2} & 3 & 18 & 3 & 5 & 24 & 17 & 11 \\
hs096 & \textbf{2} & 22 & \textbf{2} & 3 & 24 & 3 & 5 & 23 & 22 & 11 \\
hs097 & \textbf{6} & 25 & 69 & 7 & 24 & 37 & 107 & 19 & 19 & 81 \\
hs098 & \textbf{6} & 22 & 69 & 7 & 21 & 37 & 88 & 19 & 93 & 81 \\
hs099 & 61 & \textbf{6} & -- & 16 & 7 & 19 & 59 & -- & 22 & 150 \\
hs100lnp & \textbf{12} & 21 & 19 & 14 & 21 & 33 & 132 & 32 & \textbf{12} & 35 \\
hs100mod & \textbf{12} & 22 & 28 & 14 & 27 & 32 & 122 & 137 & 15 & 86 \\
hs100 & \textbf{12} & 19 & 19 & 13 & 22 & 23 & 128 & 63 & \textbf{12} & 165 \\
hs101 & \textbf{21} & 99 & 23 & 42 & 273 & 530 & -- & -- & 64 & 639 \\
hs102 & \textbf{18} & 32 & \textbf{18} & 44 & 36 & 238 & 979 & -- & 154 & 563 \\
hs103 & 1637 & 57 & \textbf{14} & 29 & 64 & 177 & 1417 & -- & 88 & 318 \\
hs104 & 25 & \textbf{10} & 34 & 26 & 11 & 29 & 84 & -- & 14 & 191 \\
hs105 & \textbf{1} & \textbf{1} & \textbf{1} & 9 & \textbf{1} & 110 & 48 & -- & 17 & \textbf{1} \\
hs106 & 16 & 16 & -- & 17 & 15 & \textbf{14} & -- & -- & 27 & 168 \\
hs107 & \textbf{6} & 11 & 8 & \textbf{6} & 12 & 14 & 19 & 26 & 35 & 102 \\
hs108 & 25 & 18 & 561 & 36 & \textbf{17} & 152 & 163 & 43 & 20 & 333 \\
hs109 & 24 & -- & 51 & \textbf{12} & 88 & 349 & -- & -- & 45 & 397 \\
hs110 & \textbf{1} & \textbf{1} & \textbf{1} & 5 & \textbf{1} & 34 & 14 & 5 & 8 & \textbf{1} \\
hs111lnp & 40 & \textbf{16} & 42 & 31 & \textbf{16} & 64 & 387 & 57 & 17 & 329 \\
hs111 & 40 & 16 & 42 & 31 & 16 & 70 & 387 & 46 & \textbf{15} & 348 \\
hs112 & \textbf{12} & 18 & \textbf{12} & 13 & 18 & 47 & 32 & 47 & 19 & 58 \\
hs113 & \textbf{6} & 13 & \textbf{6} & \textbf{6} & 12 & 28 & 145 & 97 & 17 & 193 \\
hs114 & 197 & -- & -- & 13 & 150 & \textbf{9} & -- & 664 & -- & 48 \\
hs116 & \textbf{12} & 28 & -- & 15 & 26 & 23 & 98 & -- & 24 & 164 \\
hs117 & \textbf{6} & 31 & 8 & \textbf{6} & 23 & 20 & 156 & 66 & 19 & 289 \\
hs119 & \textbf{7} & 14 & 8 & 8 & 15 & 66 & 22 & 28 & 29 & 26 \\
hs99exp & 42 & 25 & -- & 22 & 30 & 42 & 211 & -- & 256 & \textbf{3} \\
hubfit & \textbf{2} & 9 & 3 & \textbf{2} & 9 & 9 & 4 & 8 & -- & -- \\
humps & \textbf{1} & \textbf{1} & \textbf{1} & -- & \textbf{1} & 173 & 51 & -- & 307 & \textbf{1} \\
hypcir & 7 & \textbf{6} & \textbf{6} & 9 & 8 & -- & 9 & 10 & 8 & 36 \\
jensmp & \textbf{1} & \textbf{1} & \textbf{1} & 11 & \textbf{1} & 38 & 16 & 10 & 14 & \textbf{1} \\
kiwcresc & \textbf{11} & 12 & 45 & \textbf{11} & \textbf{11} & 18 & 82 & 23 & 14 & 84 \\
kowosb & \textbf{1} & \textbf{1} & \textbf{1} & 18 & \textbf{1} & 28 & 16 & 24 & 11 & \textbf{1} \\
lakes & 800 & 74 & -- & 76 & 18 & 39 & -- & -- & 288 & \textbf{1} \\
launch & 1523 & -- & -- & \textbf{164} & 1532 & 449 & -- & -- & -- & 495 \\
lewispol & 4 & -- & 5 & 4 & -- & 6 & -- & -- & -- & \textbf{1} \\
loadbal & \textbf{8} & 18 & 15 & \textbf{8} & 36 & 90 & 48 & 62 & 23 & 26 \\
loghairy & \textbf{1} & \textbf{1} & \textbf{1} & -- & -- & 135 & 90 & -- & 64 & \textbf{1} \\
logros & \textbf{1} & \textbf{1} & \textbf{1} & 50 & \textbf{1} & 173 & 56 & 66 & 398 & \textbf{1} \\
lootsma & \textbf{5} & 12 & 16 & \textbf{5} & 16 & 9 & 38 & 9 & 12 & 15 \\
lsnnodoc & 6 & 13 & \textbf{1} & 7 & 26 & 11 & 2 & 11 & 21 & 3 \\
madsen & 14 & 24 & \textbf{12} & 25 & 25 & 13 & 73 & 26 & 26 & 216 \\
makela1 & 12 & 20 & 17 & 16 & 19 & \textbf{9} & 70 & 19 & 15 & 82 \\
makela2 & \textbf{5} & 9 & 14 & \textbf{5} & 8 & 27 & 60 & 40 & 12 & 10 \\
makela3 & 22 & 18 & 29 & 25 & \textbf{17} & 51 & 239 & 125 & 18 & 81 \\
maratos & 10 & \textbf{5} & 19 & 10 & \textbf{5} & 9 & 19 & 9 & 7 & 29 \\
matrix2 & \textbf{12} & 22 & 21 & \textbf{12} & 21 & 14 & 64 & 13 & 26 & 537 \\
maxlika & \textbf{1} & \textbf{1} & \textbf{1} & 9 & \textbf{1} & 110 & 48 & -- & 17 & \textbf{1} \\
mconcon & 15 & 10 & \textbf{6} & 8 & 10 & 9 & -- & 676 & -- & 444 \\
mdhole & \textbf{1} & \textbf{1} & \textbf{1} & 56 & \textbf{1} & 98 & 41 & 68 & 98 & \textbf{1} \\
methanb8 & \textbf{1} & \textbf{1} & \textbf{1} & 47 & \textbf{1} & 720 & 84 & 221 & 155 & \textbf{1} \\
methanl8 & \textbf{1} & \textbf{1} & \textbf{1} & 96 & \textbf{1} & 1095 & 330 & 640 & 80 & \textbf{1} \\
mexhat & \textbf{1} & \textbf{1} & \textbf{1} & 10 & \textbf{1} & 35 & 5 & 4 & 7 & \textbf{1} \\
meyer3 & \textbf{1} & -- & -- & 280 & \textbf{1} & -- & 308 & 559 & 522 & \textbf{1} \\
mifflin1 & 10 & 8 & 18 & 23 & \textbf{7} & 9 & 37 & 18 & 9 & 42 \\
mifflin2 & \textbf{10} & 17 & 20 & \textbf{10} & 16 & 18 & 125 & 50 & 13 & 42 \\
minmaxbd & 50 & 115 & 20 & \textbf{9} & 78 & 72 & 357 & 592 & 31 & 1021 \\
minmaxrb & \textbf{3} & 12 & 28 & 4 & 11 & 9 & 113 & 81 & 14 & 12 \\
minsurf & \textbf{1} & \textbf{1} & \textbf{1} & 10 & \textbf{1} & 50 & 83 & 15 & 13 & \textbf{1} \\
mistake & 22 & 16 & \textbf{9} & 18 & 15 & 19 & 158 & 30 & 15 & 291 \\
mwright & \textbf{9} & 11 & 18 & 12 & 11 & 12 & 36 & 19 & 11 & 74 \\
nonmsqrt & \textbf{1} & -- & \textbf{1} & 716 & -- & -- & 489 & 167 & -- & -- \\
nuffield\footnote{full name: nuffield\_continuum, which this table is too narrow to contain.} & \textbf{5} & 8 & \textbf{5} & \textbf{5} & 7 & 10 & 6 & 15 & 10 & 17 \\
odfits & \textbf{7} & 11 & 10 & 8 & 11 & 18 & 9 & 49 & 15 & 15 \\
optcntrl & 4 & 191 & \textbf{3} & 5 & 268 & 5 & 14 & 352 & 58 & 18 \\
optmass & 9 & 26 & 812 & 19 & 46 & \textbf{2} & 330 & -- & 15 & 269 \\
optprloc & 16 & 20 & 32 & \textbf{7} & 19 & 12 & 684 & 438 & 23 & 70 \\
orthregb & \textbf{2} & 3 & 3 & \textbf{2} & 3 & 9 & 261 & 64 & 8 & \textbf{2} \\
orthrege & 2786 & 70 & -- & 180 & 79 & \textbf{31} & 856 & 795 & 482 & 13037 \\
osbornea & \textbf{1} & \textbf{1} & -- & -- & \textbf{1} & 267 & 53 & 57 & -- & \textbf{1} \\
osborneb & \textbf{1} & \textbf{1} & \textbf{1} & 20 & \textbf{1} & 120 & 60 & 45 & 19 & \textbf{1} \\
palmer1a & \textbf{1} & \textbf{1} & \textbf{1} & 51 & \textbf{1} & 385 & -- & 102 & 113 & \textbf{1} \\
palmer1b & \textbf{1} & \textbf{1} & \textbf{1} & 21 & \textbf{1} & 120 & -- & 55 & 65 & \textbf{1} \\
palmer1e & \textbf{1} & \textbf{1} & \textbf{1} & 74 & \textbf{1} & 407 & 64 & 353 & 187 & \textbf{1} \\
palmer1 & \textbf{1} & \textbf{1} & \textbf{1} & 33 & \textbf{1} & 44 & 15 & 28 & 41 & \textbf{1} \\
palmer2a & \textbf{1} & \textbf{1} & \textbf{1} & 68 & \textbf{1} & 227 & 81 & 211 & 169 & \textbf{1} \\
palmer2b & \textbf{1} & \textbf{1} & \textbf{1} & 16 & \textbf{1} & 72 & -- & 77 & 52 & \textbf{1} \\
palmer2e & \textbf{1} & \textbf{1} & \textbf{1} & 86 & \textbf{1} & 374 & 155 & 133 & 171 & \textbf{1} \\
palmer2 & \textbf{1} & \textbf{1} & \textbf{1} & 33 & \textbf{1} & 63 & -- & 34 & 24 & \textbf{1} \\
palmer3a & \textbf{1} & \textbf{1} & \textbf{1} & 82 & \textbf{1} & 267 & -- & 201 & 172 & \textbf{1} \\
palmer3b & \textbf{1} & \textbf{1} & \textbf{1} & 21 & \textbf{1} & 66 & -- & 36 & 37 & \textbf{1} \\
palmer3e & \textbf{1} & \textbf{1} & \textbf{1} & 117 & \textbf{1} & 573 & 187 & -- & 234 & \textbf{1} \\
palmer3 & \textbf{1} & \textbf{1} & \textbf{1} & 12 & \textbf{1} & 21 & 4 & 58 & 32 & \textbf{1} \\
palmer4a & \textbf{1} & \textbf{1} & \textbf{1} & 52 & \textbf{1} & 183 & -- & 93 & 110 & \textbf{1} \\
palmer4b & \textbf{1} & \textbf{1} & \textbf{1} & 21 & \textbf{1} & 61 & -- & 64 & 35 & \textbf{1} \\
palmer4e & \textbf{1} & \textbf{1} & \textbf{1} & 24 & \textbf{1} & 271 & 91 & 123 & 87 & \textbf{1} \\
palmer4 & \textbf{1} & \textbf{1} & \textbf{1} & 12 & \textbf{1} & 21 & 4 & 142 & 35 & \textbf{1} \\
palmer5a & -- & -- & -- & -- & -- & -- & \textbf{112071} & -- & -- & -- \\
palmer5b & \textbf{1} & \textbf{1} & \textbf{1} & 855 & \textbf{1} & -- & 1513 & 961 & -- & -- \\
palmer5e & \textbf{1} & -- & -- & 3 & -- & -- & 10615 & 8 & -- & -- \\
palmer6a & \textbf{1} & \textbf{1} & \textbf{1} & 137 & \textbf{1} & 355 & 117 & 277 & -- & -- \\
palmer6e & \textbf{1} & \textbf{1} & \textbf{1} & 38 & \textbf{1} & 407 & 114 & 47 & -- & -- \\
palmer7a & \textbf{1} & -- & \textbf{1} & -- & -- & -- & -- & -- & -- & -- \\
palmer7e & \textbf{1} & -- & -- & -- & -- & -- & 332 & 39 & -- & -- \\
palmer8a & \textbf{1} & \textbf{1} & \textbf{1} & 50 & \textbf{1} & 192 & 43 & 61 & -- & -- \\
palmer8e & \textbf{1} & \textbf{1} & \textbf{1} & 29 & \textbf{1} & 213 & 49 & 86 & -- & -- \\
pentagon & 8 & 20 & 9 & 13 & 20 & 20 & \textbf{5} & 48 & 38 & 23 \\
pfit1ls & \textbf{1} & \textbf{1} & \textbf{1} & 566 & \textbf{1} & 784 & 286 & 453 & 337 & \textbf{1} \\
pfit1 & \textbf{1} & \textbf{1} & \textbf{1} & 566 & \textbf{1} & 784 & 286 & 453 & 337 & \textbf{1} \\
pfit2ls & \textbf{1} & \textbf{1} & \textbf{1} & 210 & \textbf{1} & 283 & 83 & 217 & 115 & \textbf{1} \\
pfit2 & \textbf{1} & \textbf{1} & \textbf{1} & 210 & \textbf{1} & 283 & 83 & 217 & 115 & \textbf{1} \\
pfit3ls & \textbf{1} & \textbf{1} & \textbf{1} & 139 & \textbf{1} & 506 & 181 & 272 & 148 & \textbf{1} \\
pfit3 & \textbf{1} & \textbf{1} & \textbf{1} & 139 & \textbf{1} & 506 & 181 & 272 & 148 & \textbf{1} \\
pfit4ls & \textbf{1} & \textbf{1} & \textbf{1} & 126 & \textbf{1} & 881 & 290 & 410 & 286 & \textbf{1} \\
pfit4 & \textbf{1} & \textbf{1} & \textbf{1} & 126 & \textbf{1} & 881 & 290 & 410 & 286 & \textbf{1} \\
polak1 & 8 & 8 & 15 & 8 & \textbf{7} & 18 & 87 & 37 & 14 & 97 \\
polak2 & 55 & 30 & 450 & 34 & 28 & 226 & 351 & 321 & \textbf{24} & 816 \\
polak3 & 26 & -- & 18 & 43 & -- & 209 & -- & 234 & 24 & \textbf{3} \\
polak4 & \textbf{5} & 11 & 9 & \textbf{5} & 7 & 7 & 77 & 16 & 11 & 153 \\
polak5 & 96 & 34 & 192 & 88 & 33 & 59 & 69 & \textbf{7} & 69 & 32 \\
polak6 & 40 & -- & 47 & 29 & 316 & 109 & 249 & 644 & \textbf{27} & 206 \\
powellbs & 116 & \textbf{12} & 196 & 16 & \textbf{12} & -- & 16 & -- & 17 & 252 \\
powellsq & 521 & -- & -- & 24 & 116 & 218 & -- & \textbf{23} & -- & 42 \\
prodpl0 & \textbf{9} & 17 & 12 & 10 & 32 & 15 & 42 & 35 & 24 & 350 \\
prodpl1 & \textbf{7} & 18 & 16 & 8 & 34 & 11 & 71 & 27 & 21 & 280 \\
pspdoc & \textbf{1} & \textbf{1} & \textbf{1} & 7 & \textbf{1} & 14 & 11 & 10 & 12 & \textbf{1} \\
recipe & \textbf{2} & 3 & 3 & 3 & 3 & -- & 4 & 12 & 10 & 3 \\
rk23 & \textbf{9} & 11 & 19 & 10 & 12 & 12 & 59 & 54 & 12 & 178 \\
robot & 20 & 11 & 1192 & 45 & \textbf{10} & 18 & 376 & 33 & 18 & 592 \\
rosenbr & \textbf{1} & \textbf{1} & \textbf{1} & 29 & \textbf{1} & 62 & 2 & 36 & 26 & \textbf{1} \\
rosenmmx & 39 & 42 & 24 & 39 & 47 & 42 & 168 & 226 & \textbf{17} & 495 \\
s365mod & 29 & -- & 14890 & 108 & 43 & 31 & 538 & -- & \textbf{28} & 581 \\
sineali & \textbf{1} & -- & \textbf{1} & -- & -- & -- & 3266 & -- & 16 & \textbf{1} \\
sineval & \textbf{1} & \textbf{1} & \textbf{1} & 62 & \textbf{1} & 120 & 47 & 75 & 57 & \textbf{1} \\
sisser & \textbf{1} & \textbf{1} & \textbf{1} & 19 & \textbf{1} & 13 & 5 & 38 & 17 & \textbf{1} \\
snake & \textbf{3} & -- & 99 & \textbf{3} & 14 & 7 & 22 & -- & -- & 6 \\
spanhyd & 4 & 24 & \textbf{2} & 12 & 22 & 93 & -- & 26 & -- & 24 \\
spiral & 122 & -- & 623 & 152 & \textbf{64} & 108 & 393 & 96 & 135 & 3427 \\
ssnlbeam & \textbf{5} & 31 & 64 & 6 & 22 & 36 & 123 & 39 & 60 & 212 \\
stancmin & \textbf{1} & 12 & 2 & 3 & 11 & 5 & 2 & 9 & 20 & 5 \\
swopf & \textbf{5} & 18 & -- & 7 & 34 & 25 & 138 & 290 & 21 & 100 \\
synthes1 & \textbf{5} & 11 & \textbf{5} & \textbf{5} & 10 & 10 & 20 & 13 & 17 & 88 \\
try-b & \textbf{8} & 20 & 9 & \textbf{8} & 20 & 10 & 10 & 13 & 16 & 28 \\
twobars & \textbf{8} & 11 & 12 & \textbf{8} & 10 & 11 & 30 & 13 & 10 & 87 \\
vanderm4 & \textbf{17} & -- & 22 & 22 & 102 & 58 & -- & 36 & -- & 105 \\
watson & \textbf{1} & \textbf{1} & \textbf{1} & 21 & \textbf{1} & 356 & 49 & 44 & 18 & \textbf{1} \\
weeds & \textbf{1} & \textbf{1} & \textbf{1} & 39 & \textbf{1} & 77 & -- & 3 & 29 & \textbf{1} \\
womflet & 46 & 14 & 3783 & \textbf{9} & 12 & 28 & 136 & 97 & 12 & 137 \\
yfit & \textbf{1} & \textbf{1} & \textbf{1} & 48 & \textbf{1} & 154 & 60 & 103 & 45 & \textbf{1} \\
yfitu & \textbf{1} & \textbf{1} & \textbf{1} & 48 & \textbf{1} & 154 & 60 & 103 & 43 & \textbf{1} \\
zecevic3 & 15 & 23 & 340 & 12 & 22 & \textbf{11} & 37 & 19 & 12 & 173 \\
zecevic4 & \textbf{6} & 11 & \textbf{6} & 7 & 10 & 8 & 21 & 12 & 15 & 77 \\
zigzag & \textbf{11} & 28 & 76 & 12 & 46 & 23 & 217 & 43 & 29 & 525 \\
zy2 & \textbf{5} & 13 & 16 & \textbf{5} & 10 & 9 & 43 & 9 & 14 & 16 \\
\hline
\end{longtable}
\end{scriptsize}



==> sections/sufficient_decrease.tex <==
\section{Unifying sufficient decrease conditions}

\begin{landscape}
\begin{table}[htbp!]
\centering
\scriptsize
\begin{tabular}{|p{3.1cm}|p{15.2cm}|}
\hline
Subproblem              & Mathematical definition \\
\hline
\multirow{3}{*}{Optimality QP}   &
$\begin{array}{ll} \dps
\mini_d &
\frac{1}{2} d^T W_1^{(k)}(x^{(k)}, \constraintmultipliers^{(k)}) d + 1 \nabla (f^{(k)})^T d \\
\st 	& c^{(k)} + (\nabla c^{(k)})^T d = 0 \\
      & x^{(k)} + d \ge 0
\end{array}$
\\
\cline{2-2}
   & Merit function (\charlie{requires $\rho$ steered}): \newline
   $(\rho f(x^{(k)}) + \|c(x^{(k)})\|_1) - (\rho f(x^{(k+1)}) + \|c(x^{(k+1)})\|_1) \ge \sigma \left(\| c^{(k)} \|_1 - \rho (\nabla f^{(k)})^T d - \| c^{(k)} + (\nabla c^{(k)})^T d \|_1 \right)$  \\
\cline{2-2}
   & Filter: $f(x^{(k)}) - f(x^{(k+1)}) \ge \sigma \left(-(\nabla f^{(k)})^T d \right)$ \\
\hline
\multirow{3}{*}{$\ell_1$QP with $\rho > 0$}  &
$\begin{array}{ll} \dps
\mini_d &
\frac{1}{2} d^T W_\rho(x^{(k)}, \constraintmultipliers^{(k)}) d + \rho (\nabla f^{(k)})^T d
%\frac{1}{2} d^T \zeta D^2 d + \zeta D^2 (x^{(k)} - x)^T d
 +
\| c^{(k)} + (\nabla c^{(k)})^T d \|_1 \\
\st 	& x^{(k)} + d \ge 0
\end{array}$
\\
\cline{2-2}
   & Merit function:
   $\left( \rho f(x^{(k)}) + \|c(x^{(k)})\|_1 \right) -
   \left( \rho f(x^{(k+1)}) +
   %\frac{\zeta}{2} \|D (x^{(k+1)} - x^{(k)}) \|^2_2 +
   \|c(x^{(k+1)})\|_1 \right) \ge
   \sigma \left(
   \| c^{(k)} \|_1 - \rho (\nabla f^{(k)})^T d
   %- \frac{1}{2} d^T \zeta D^2 d - \zeta D^2 (x^{(k)} - x)^T d
   - \| c^{(k)} + (\nabla c^{(k)})^T d \|_1 \right)$ \\
\cline{2-2}
   & Filter: \quad
   $f(x^{(k)}) - f(x^{(k+1)})
   \ge
   \sigma \left(
   -(\nabla f^{(k)})^T d
   %- \frac{1}{2} d^T \zeta D^2 d - \zeta D^2 (x^{(k)} - x)^T d
   \right)$
   %\charlie{ii) if $\rho = 0$, filter condition not relevant. $\objectivemeasure$ redefined (a la filterSQP)}
   \\
\hline
$\ell_1$QP with $\rho = 0$ \newline (feasibility QP) \newline \charlie{redefine $(\omega, \eta) = (\eta, 0)$}  &
$\begin{array}{ll} \dps
\mini_d &
\frac{1}{2} d^T W_0(x^{(k)}, \constraintmultipliers^{(k)}) d + \| c^{(k)} + (\nabla c^{(k)})^T d \|_1 \\
\st 	& x^{(k)} + d \ge 0
\end{array}$ \\
\cline{2-2}
   & Merit function: \quad $\|c(x^{(k)})\|_1 - \|c(x^{(k+1)})\|_1 \ge \sigma \left(\| c^{(k)} \|_1 - \| c^{(k)} + (\nabla c^{(k)})^T d \|_1 \right)$ \\
\cline{2-2}
   & Filter: \quad $\|c(x^{(k)})\|_1 - \|c(x^{(k+1)})\|_1 \ge \sigma \left(\| c^{(k)} \|_1 - \| c^{(k)} + (\nabla c^{(k)})^T d \|_1 \right)$ \quad \\
\hline
%\hline
%Bound-constrained AL QP &
%$\begin{array}{ll} \dps
%\mini_d & \frac{1}{2} d^T W_\rho(x^{(k)}, \rho \constraintmultipliers^{(k)} - c^{(k)}) d + \rho ((\nabla f^{(k)})^T d - \nabla c^{(k)} y^{(k)}) + \frac{1}{2} d^T \nabla c^{(k)} (\nabla c^{(k)})^T d + \nabla c^{(k)} (c^{(k)})^T d \\
%\st 	& x^{(k)} + d \ge 0
%\end{array}$
%\\
\hline
\multirow{3}{*}{Optimality barrier}   &
$\begin{array}{ll} \dps
\mini_d &
\frac{1}{2} d^T W_1(x^{(k)}, \constraintmultipliers^{(k)}) d + (\nabla f^{(k)})^T d + \frac{1}{2} d^T (X^{(k)})^{-1} Z^{(k)} d - \mu (X^{(k)})^{-1} e^T d \\
\st 	& c^{(k)} + (\nabla c^{(k)})^T d = 0
\end{array}$
\\
\cline{2-2}
   & Merit function: (\charlie{requires $\rho$ steered}) \newline
   $(\rho f(x^{(k)}) + \|c(x^{(k)})\|_1 - \mu \log(X^{(k)}) e) - (\rho f(x^{(k+1)}) + \|c(x^{(k+1)})\|_1 - \mu \log(X^{(k+1)}) e) \ge \newline \sigma \left(\| c^{(k)} \|_1 - \rho (\nabla f^{(k)})^T d - \| c^{(k)} + (\nabla c^{(k)})^T d \|_1 + \mu (X^{(k)})^{-1} e^T d \right)$ \\
\cline{2-2}
   & Filter:
   $(f(x^{(k)}) - \mu \log(X^{(k)}) e) - (f(x^{(k+1)}) - \mu \log(X^{(k+1)}) e) \ge \sigma \left(- (\nabla f^{(k)})^T d + \mu (X^{(k)})^{-1} e^T d \right)$ \\
\hline
\multirow{3}{*}{$\ell_1$ interior-point with $\rho > 0$}   &
$\begin{array}{ll} \dps
\mini_d &
\frac{1}{2} d^T W_\rho(x^{(k)}, \constraintmultipliers^{(k)}) d + \rho (\nabla f^{(k)})^T d
% \frac{1}{2} d^T \zeta D^2 d + \zeta D^2 (x^{(k)} - x)^T d +
\| c^{(k)} + (\nabla c^{(k)})^T d \|_1 +
\frac{1}{2} d^T (X^{(k)})^{-1} Z^{(k)} d - \mu (X^{(k)})^{-1} e^T d
\end{array}$
\\
\cline{2-2}
   & Merit function: \newline
   $(\rho f(x^{(k)}) + \|c(x^{(k)})\|_1 - \mu \log(X^{(k)}) e) - (\rho f(x^{(k+1)}) + \|c(x^{(k+1)})\|_1 - \mu \log(X^{(k+1)}) e) \ge \newline \sigma \left( \| c^{(k)} \|_1 - \rho (\nabla f^{(k)})^T d - \| c^{(k)} + (\nabla c^{(k)})^T d \|_1 + \mu (X^{(k)})^{-1} e^T d \right)$ \\
\cline{2-2}
   & Filter:
   $(f(x^{(k)}) - \mu \log(X^{(k)}) e) - (f(x^{(k+1)}) - \mu \log(X^{(k+1)}) e) \ge \sigma \left(-(\nabla f^{(k)})^T d + \mu (X^{(k)})^{-1} e^T d \right)$ \\
\hline
$\ell_1$ interior-point with $\rho = 0$ \newline (feasibility interior-point) \newline \charlie{redefine $(\omega, \eta) = (\eta, 0)$} &
$\begin{array}{ll} \dps
\mini_d &
\frac{1}{2} d^T W_0(x^{(k)}, \constraintmultipliers^{(k)}) d + \| c^{(k)} + (\nabla c^{(k)})^T d \|_1 + \frac{1}{2} d^T (X^{(k)})^{-1} Z^{(k)} d - \mu (X^{(k)})^{-1} e^T d
\end{array}$ \\
\cline{2-2}
   & Merit function: \newline
   $(\|c(x^{(k)})\|_1 - \mu \log(X^{(k)}) e) - (\|c(x^{(k+1)})\|_1 - \mu \log(X^{(k+1)}) e) \ge \sigma \left(\| c^{(k)} \|_1 - \| c^{(k)} + (\nabla c^{(k)})^T d \|_1 + \mu (X^{(k)})^{-1} e^T d \right)$ \\
\cline{2-2}
   & Filter: \newline
   $(\|c(x^{(k)})\|_1 - \mu \log(X^{(k)}) e) - (\|c(x^{(k+1)})\|_1 - \mu \log(X^{(k+1)}) e) \ge \sigma \left(\| c^{(k)} \|_1 - \| c^{(k)} + (\nabla c^{(k)})^T d \|_1 + \mu (X^{(k)})^{-1} e^T d \right)$ \quad  \\
\hline
%Bound-constrained interior-point AL  &
%$\begin{array}{ll} \dps
%\mini_d & \frac{1}{2} d^T W_\rho(x^{(k)}, \rho \constraintmultipliers^{(k)} - c^{(k)}) d + \rho ((\nabla f^{(k)})^T d - \nabla c^{(k)} y^{(k)}) + \frac{1}{2} d^T \nabla c^{(k)} (\nabla c^{(k)})^T d + \nabla c^{(k)} (c^{(k)})^T d + \frac{1}{2} d^T (X^{(k)})^{-1} Z^{(k)} d - \mu (X^{(k)})^{-1} e^T d
%\end{array}$
%\\
%\hline
\end{tabular}
\end{table}
\end{landscape}

